Is my transaction done yet? An empirical study of transaction processing times in the Ethereum Blockchain Platform

Ethereum is one of the most popular platforms for the development of blockchain-powered applications. These applications are known as Dapps. When engineering Dapps, developers need to translate requests captured in the front-end of their application into one or more smart contract transactions. Developers need to pay for these transactions and, the more they pay (i.e., the higher the gas price), the faster the transaction is likely to be processed. Therefore developers need to optimize the balance between cost (transaction fees) and user experience (transaction processing times). Online services have been developed to provide transaction issuers (e.g., Dapp developers) with an estimate of how long transactions will take to be processed given a certain gas price. These estimation services are crucial in the Ethereum domain and several popular wallets such as Metamask rely on them. However, their accuracy has not been empirically investigated so far. In this paper, we quantify the transaction processing times in Ethereum, investigate the relationship between processing times and gas prices, and determine the accuracy of state-of-the-practice estimation services. We find that transactions are processed in a median of 57s and that 90% of the transactions are processed within 8m. The higher gas prices result in faster transaction processing times with diminishing returns. In particular, we observe no practical difference in processing time between expensive and very expensive transactions. In terms of accuracy of processing time estimation services, we note that they are equivalent. However, when stratifying transactions by gas prices, Etherscan's Gas Tracker is the most accurate estimation service for very cheap and cheap transaction. EthGasStation's Gas Price API, in turn, is the most accurate estimation service for regular, expensive, and very expensive transactions.

==> bios.tex <==
\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/mike.png}}]{Michael Pacheco} is a MSc student at the School of Computing of Queen's University in Canada under the supervision of Dr. Ahmed Hassan and Dr. Gustavo A. Oliva. His research at the Software Analysis and Intelligence Lab (SAIL) focuses on understanding and evaluating the transaction processing mechanism of Ethereum.
\end{IEEEbiography}
		
\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/gus.png}}]
	{Gustavo A. Oliva} is a Research Fellow at the School of Computing of Queen's University in Canada under the supervision of professor Dr. Ahmed E. Hassan. Gustavo leads the blockchain research team at the Software Analysis and Intelligence Lab (SAIL). In his research, Gustavo leverages his expertise on software architecture, social network analysis, and machine learning to analyze blockchain with Software Engineering lens. Gustavo received his MSc and PhD degrees from the University of São Paulo (USP) in Brazil under the supervision of professor Dr. Marco Aurélio Gerosa. More information at: \url{https://www.gaoliva.com}
\end{IEEEbiography}

\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/gopi.jpg}}] {Gopi Krishnan Rajbahadur} is currently a Ph.D. student in the Software Analysis and Intelligence Lab (SAIL) at Queen’s University, Canada. He received his BE in computer Science and Engineering from SKR Engineering college, Anna University, India. He also spent close to five years working as a data scientist in various software corporations in both India and Canada. His research interests include interpretable machine learning, mining software repositories and safe data science. More information at: \url{http://gopikrishnanrajbahadur.me}
\end{IEEEbiography}
	
\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/ahmed.png}}] {Ahmed E. Hassan} is an IEEE Fellow, an ACM SIGSOFT Influential	Educator, an NSERC Steacie Fellow, the Canada Research Chair (CRC) in Software Analytics, and the NSERC/BlackBerry Software Engineering Chair at the School of Computing at Queen’s University, Canada. His research interests include mining software repositories, empirical software engineering, load testing, and log mining. He received a PhD in Computer Science from the University of Waterloo. He spearheaded the creation of the Mining Software Repositories (MSR) conference and its research community. He also serves/d on the editorial boards of IEEE Transactions on Software Engineering, Springer Journal of Empirical Software Engineering, and PeerJ Computer Science. Contact ahmed@cs.queensu.ca. More information at: \url{http://sail.cs.queensu.ca}.
\end{IEEEbiography}

==> extra.tex <==
Moreover, very limited information is provided regarding the design and validation of these models, making it unclear what factors influence processing time the most. Finally, designing a new model that outperforms the predictions produced by these state-of-the-practice tools has the potential to drastically improve the economics behind \dapps. 

-----------------

Finally we investigate how network utilization influences transaction processing times. We quantify network utilization using the following metric:

\begin{scriptsize}
\begin{equation}
    \begin{aligned}
      NetworkUtilization(B_i, t) = \dfrac{\sum_{i-t}^{i-1}BlockFilledPercentage(B_i)}{t} \\
      BlockFilledPercentage(B) = \dfrac{gasUsed(B)}{gasLimit(B)} * 100
    \end{aligned}
\end{equation}
\end{scriptsize}

As shown above, the network utilization metric is a function of the $BlockFilledPercentage(B)$ metric. $BlockFilledPercentage(B)$ is defined as the ratio between the \textit{block gas used} over the \textit{block gas limit} of a given block $B$. The network utilization is then defined as taking the average of $BlockFilledPercentage$ over the \textit{t} blocks that were appended before block $B_i$, where \textit{i} denotes the \textit{block number}. We use $t = 120$ for this project, which in units of time represents approximately 30 minutes (as it is assumed that the Ethereum blockchain appends a new block to the chain every 15 seconds).

\smallskip \observation{Cheaper transactions are more susceptible to delays in processing time when the network utilization increases.} Figure \ref{fig:net_cong} depicts a heatmap in which we compare the median processing time per block (i.e., the median of the processing times of all transactions in a given block) with the network utilization. A visual inspection of the heatmap indicates that most of the observations lie in the upper left corner of the figure (note the red hexagons), with no apparent correlation between the two variables. Indeed, the Spearman's rho indicates that there is only very weak (0.05) correlation between them.

\begin{figure}[!htbp]
\centering
  \includegraphics[width=\linewidth]{rq1/net_cong_vs_median_pr_time.pdf}
  \caption{Heatmap contrasting the median transaction processing time per block with the network utilization level.}
  \label{fig:net_cong}
\end{figure}

We conjecture that network utilization impacts only transactions with cheaper prices. Therefore, we investigated how processing times vary for different price categories and different network utilization levels. The results are depicted in Figure \ref{fig:net_cong_range_vs_med_pr_time}. The figure corroborates our conjecture. As network utilization increases, the processing time of cheaper transactions tends to increase (e.g., note the red boxplots and their medians). Expensive and very expensive transactions are remarkably less impacted by network utilization. Interestingly, for all gas price categories, the median processing time of transactions is lower for an utilization level of (90, 100] compared to the (80, 90] utilization level. We hypothesize that miner nodes start working more intensively when the network is being very highly utilized (e.g., when it shows first signs of congestion).

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{rq1/net_cong_vs_price_category.pdf}
    \caption{Relation between network utilization on gas prices}
    \label{fig:net_cong_range_vs_med_pr_time}
\end{figure}


